Design and Analysis of a Logless Dynamic Reconfiguration Protocol

Distributed replication systems based on the replicated state machine model have become ubiquitous as the foundation of modern database systems. To ensure availability in the presence of faults, these systems must be able to dynamically replace failed nodes with healthy ones via dynamic reconfiguration. MongoDB is a document oriented database with a distributed replication mechanism derived from the Raft protocol. In this paper, we present MongoRaftReconfig, a novel dynamic reconfiguration protocol for the MongoDB replication system. MongoRaftReconfig utilizes a logless approach to managing configuration state and decouples the processing of configuration changes from the main database operation log. The protocol's design was influenced by engineering constraints faced when attempting to redesign an unsafe, legacy reconfiguration mechanism that existed previously in MongoDB. We provide a safety proof of MongoRaftReconfig, along with a formal specification in TLA+. To our knowledge, this is the first published safety proof and formal specification of a reconfiguration protocol for a Raft-based system. We also present results from model checking its safety properties on finite protocol instances. Finally, we discuss the conceptual novelties of MongoRaftReconfig, how it can be understood as an optimized and generalized version of the single server reconfiguration algorithm of Raft, and present an experimental evaluation of how its optimizations can provide performance benefits for reconfigurations.

==> figures/cex-tikz/elecsafety-no-config-check.tex <==
\begin{tabular}{c|c|c|c|c|c|c}
 & $1$ & $2$ & $3$ & $4$ & $5$ & $6$\\ \hline 

$n_0$ & $\underset{\underset{}{\{n_1,n_2,n_3\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{}{\{n_1,n_2,n_3\}}}{P^{1 \, \textcolor{blue}{\symqueen}}_{(1,1)}}$ & $\underset{\underset{}{\{n_1,n_2\}}}{P^{1 \, \textcolor{blue}{\symqueen}}_{(2,1)}}$ & $\underset{\underset{}{\{n_1\}}}{P^{1 \, \textcolor{blue}{\symqueen}}_{(3,1)}}$ & $\underset{\underset{}{\{n_1\}}}{P^{2 \, \textcolor{blue}{\symqueen}}_{(3,2)}}$ & \cellcolor{red!10}$\underset{\underset{}{\{n_1\}}}{P^{2 \, \textcolor{blue}{\symqueen}}_{(3,2)}}$\\
 

$n_1$ & $\underset{\underset{}{\{n_1,n_2,n_3\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{}{\{n_1,n_2,n_3\}}}{S^{1 \, }_{(1,0)}}$ & $\underset{\underset{}{\{n_1,n_2,n_3\}}}{S^{1 \, }_{(1,0)}}$ & $\underset{\underset{}{\{n_1,n_2,n_3\}}}{S^{1 \, }_{(1,0)}}$ & $\underset{\underset{}{\{n_1,n_2,n_3\}}}{S^{1 \, }_{(1,0)}}$ & \cellcolor{red!10}$\underset{\underset{}{\{n_1,n_2,n_3\}}}{P^{2 \, \textcolor{blue}{\symqueen}}_{(1,2)}}$\\
 

$n_2$ & $\underset{\underset{}{\{n_1,n_2,n_3\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{}{\{n_1,n_2,n_3\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{}{\{n_1,n_2,n_3\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{}{\{n_1,n_2,n_3\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{}{\{n_1,n_2,n_3\}}}{S^{0 \, }_{(1,0)}}$ & \cellcolor{red!10}$\underset{\underset{}{\{n_1,n_2,n_3\}}}{S^{2 \, }_{(1,0)}}$
\end{tabular}



==> figures/cex-tikz/elecsafety-no-term-check.tex <==
\begin{tabular}{c|c|c|c|c|c|c|c}
 & $1$ & $2$ & $3$ & $4$ & $5$ & $6$ & $7$\\ \hline 

$n_0$ & $\underset{\underset{}{\{n_1\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{}{\{n_1\}}}{P^{1 \, \textcolor{blue}{\symqueen}}_{(1,1)}}$ & $\underset{\underset{}{\{n_1,n_2\}}}{P^{1 \, \textcolor{blue}{\symqueen}}_{(2,1)}}$ & $\underset{\underset{}{\{n_1,n_2\}}}{P^{1 \, \textcolor{blue}{\symqueen}}_{(2,1)}}$ & $\underset{\underset{}{\{n_1,n_2,n_3\}}}{P^{1 \, \textcolor{blue}{\symqueen}}_{(3,1)}}$ & $\underset{\underset{}{\{n_1,n_2,n_3\}}}{P^{1 \, \textcolor{blue}{\symqueen}}_{(3,1)}}$ & \cellcolor{red!10}$\underset{\underset{}{\{n_1,n_2,n_3\}}}{P^{1 \, \textcolor{blue}{\symqueen}}_{(3,1)}}$\\
 

$n_1$ & $\underset{\underset{}{\{n_1\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{}{\{n_1\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{}{\{n_1\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{}{\{n_1,n_2\}}}{S^{0 \, }_{(2,1)}}$ & $\underset{\underset{}{\{n_1,n_2\}}}{S^{0 \, }_{(2,1)}}$ & $\underset{\underset{}{\{n_1,n_2,n_3\}}}{S^{0 \, }_{(3,1)}}$ & \cellcolor{red!10}$\underset{\underset{}{\{n_1,n_2,n_3\}}}{P^{1 \, \textcolor{blue}{\symqueen}}_{(3,1)}}$\\
 

$n_2$ & $\underset{\underset{}{\{n_1\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{}{\{n_1\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{}{\{n_1\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{}{\{n_1\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{}{\{n_1\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{}{\{n_1\}}}{S^{0 \, }_{(1,0)}}$ & \cellcolor{red!10}$\underset{\underset{}{\{n_1\}}}{S^{1 \, }_{(1,0)}}$
\end{tabular}



==> figures/cex-tikz/leadercompl-no-log-prop.tex <==
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
 & $1$ & $2$ & $3$ & $4$ & $5$ & $6$ & $7$ & $8$ & $9$ & $10$\\ \hline 

$n_0$ & $\underset{\underset{[]}{\{n_1\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{[]}{\{n_1\}}}{P^{1 \, \textcolor{blue}{\symqueen}}_{(1,1)}}$ & $\underset{\underset{[1]}{\{n_1\}}}{P^{1 \, \textcolor{blue}{\symqueen}}_{(1,1)}}$ & $\underset{\underset{[1]}{\{n_1\}}}{P^{1 \, \textcolor{blue}{\symqueen}}_{(1,1)}}$ & $\underset{\underset{[1]}{\{n_1,n_2\}}}{P^{1 \, \textcolor{blue}{\symqueen}}_{(2,1)}}$ & $\underset{\underset{[1]}{\{n_1,n_2\}}}{P^{1 \, \textcolor{blue}{\symqueen}}_{(2,1)}}$ & $\underset{\underset{[1]}{\{n_1,n_2\}}}{P^{1 \, \textcolor{blue}{\symqueen}}_{(2,1)}}$ & $\underset{\underset{[1]}{\{n_1,n_2,n_3\}}}{P^{1 \, \textcolor{blue}{\symqueen}}_{(3,1)}}$ & $\underset{\underset{[1]}{\{n_1,n_2,n_3\}}}{P^{1 \, \textcolor{blue}{\symqueen}}_{(3,1)}}$ & \cellcolor{red!10}$\underset{\underset{[1]}{\{n_1,n_2,n_3\}}}{P^{1 \, \textcolor{blue}{\symqueen}}_{(3,1)}}$\\
 

$n_1$ & $\underset{\underset{[]}{\{n_1\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{[]}{\{n_1\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{[]}{\{n_1\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{[]}{\{n_1\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{[]}{\{n_1\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{[]}{\{n_1,n_2\}}}{S^{0 \, }_{(2,1)}}$ & $\underset{\underset{[]}{\{n_1,n_2\}}}{S^{1 \, }_{(2,1)}}$ & $\underset{\underset{[]}{\{n_1,n_2\}}}{S^{1 \, }_{(2,1)}}$ & $\underset{\underset{[]}{\{n_1,n_2,n_3\}}}{S^{1 \, }_{(3,1)}}$ & \cellcolor{red!10}$\underset{\underset{[]}{\{n_1,n_2,n_3\}}}{P^{2 \, \textcolor{blue}{\symqueen}}_{(3,2)}}$\\
 

$n_2$ & $\underset{\underset{[]}{\{n_1\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{[]}{\{n_1\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{[]}{\{n_1\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{[]}{\{n_1\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{[]}{\{n_1\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{[]}{\{n_1\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{[]}{\{n_1\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{[]}{\{n_1\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{[]}{\{n_1\}}}{S^{0 \, }_{(1,0)}}$ & \cellcolor{red!10}$\underset{\underset{[]}{\{n_1\}}}{S^{2 \, }_{(1,0)}}$
\end{tabular}



==> figures/cex-tikz/leadercompl-no-term-check.tex <==
\begin{tabular}{c|c|c|c|c|c|c|c|c|c}
 & $1$ & $2$ & $3$ & $4$ & $5$ & $6$ & $7$ & $8$ & $9$\\ \hline 

$n_0$ & $\underset{\underset{[]}{\{n_1,n_2,n_3\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{[]}{\{n_1,n_2,n_3\}}}{P^{1 \, \textcolor{blue}{\symqueen}}_{(1,1)}}$ & $\underset{\underset{[1]}{\{n_1,n_2,n_3\}}}{P^{1 \, \textcolor{blue}{\symqueen}}_{(1,1)}}$ & $\underset{\underset{[1]}{\{n_1,n_2,n_3\}}}{P^{1 \, \textcolor{blue}{\symqueen}}_{(1,1)}}$ & $\underset{\underset{[1]}{\{n_1,n_3\}}}{P^{1 \, \textcolor{blue}{\symqueen}}_{(2,1)}}$ & $\underset{\underset{[1]}{\{n_1,n_3\}}}{P^{1 \, \textcolor{blue}{\symqueen}}_{(2,1)}}$ & $\underset{\underset{[1]}{\{n_1,n_3\}}}{P^{1 \, \textcolor{blue}{\symqueen}}_{(2,1)}}$ & $\underset{\underset{[1]}{\{n_1\}}}{P^{1 \, \textcolor{blue}{\symqueen}}_{(3,1)}}$ & \cellcolor{red!10}$\underset{\underset{[1]}{\{n_1\}}}{P^{1 \, \textcolor{blue}{\symqueen}}_{(3,1)}}$\\
 

$n_1$ & $\underset{\underset{[]}{\{n_1,n_2,n_3\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{[]}{\{n_1,n_2,n_3\}}}{S^{1 \, }_{(1,0)}}$ & $\underset{\underset{[]}{\{n_1,n_2,n_3\}}}{S^{1 \, }_{(1,0)}}$ & $\underset{\underset{[]}{\{n_1,n_2,n_3\}}}{S^{1 \, }_{(1,1)}}$ & $\underset{\underset{[]}{\{n_1,n_2,n_3\}}}{S^{1 \, }_{(1,1)}}$ & $\underset{\underset{[]}{\{n_1,n_2,n_3\}}}{P^{2 \, \textcolor{blue}{\symqueen}}_{(1,2)}}$ & $\underset{\underset{[]}{\{n_1,n_2,n_3\}}}{P^{2 \, \textcolor{blue}{\symqueen}}_{(1,2)}}$ & $\underset{\underset{[]}{\{n_1,n_2,n_3\}}}{P^{2 \, \textcolor{blue}{\symqueen}}_{(1,2)}}$ & \cellcolor{red!10}$\underset{\underset{[]}{\{n_1,n_2,n_3\}}}{P^{2 \, \textcolor{blue}{\symqueen}}_{(1,2)}}$\\
 

$n_2$ & $\underset{\underset{[]}{\{n_1,n_2,n_3\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{[]}{\{n_1,n_2,n_3\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{[]}{\{n_1,n_2,n_3\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{[]}{\{n_1,n_2,n_3\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{[]}{\{n_1,n_2,n_3\}}}{S^{0 \, }_{(1,0)}}$ & $\underset{\underset{[]}{\{n_1,n_2,n_3\}}}{S^{2 \, }_{(1,0)}}$ & $\underset{\underset{[]}{\{n_1,n_3\}}}{S^{2 \, }_{(2,1)}}$ & $\underset{\underset{[]}{\{n_1,n_3\}}}{S^{2 \, }_{(2,1)}}$ & \cellcolor{red!10}$\underset{\underset{[]}{\{n_1,n_3\}}}{S^{2 \, }_{(2,1)}}$
\end{tabular}



==> figures/cex-trace-elecsafety.tex <==

\begin{figure}
    \footnotesize

    %%% Figure A.
    \begin{subfigure}[b]{0.98\textwidth}
        \centering
        \input{figures/cex-tikz/elecsafety-no-config-check}                
        \caption{Safety counterexample when precondition Q1 is disabled. Proper term propagation, but insufficient config deactivation. }
        \label{fig:elecsafety-cex-a}
    \end{subfigure}\\

    %%% Figure B.
    \begin{subfigure}[b]{0.98\textwidth}
        \centering
        \input{figures/cex-tikz/elecsafety-no-term-check}
        \caption{Safety counterexample when precondition P2 is disabled. Proper config deactivation, but insufficient term propagation.}
        \label{fig:elecsafety-cex-b}
    \end{subfigure}

    \caption{\textit{OnePrimaryPerTerm} counterexamples generated by TLC. Primary servers are annotated with a \textcolor{blue}{\symqueen}. The state violating the safety property is highlighted in red. \mytodo{Adjust formatting to make figure width fit easily on page.} \mytodo{Explain server state representation.}}
\end{figure}

==> figures/cex-trace-leader-completeness.tex <==

\begin{figure}
    \footnotesize

    %%% Figure A.
    \begin{subfigure}[b]{0.98\textwidth}
        \centering
        \input{figures/cex-tikz/leadercompl-no-log-prop}
        \caption{Safety counterexample generated after disabling precondition P1. Proper term deactivation, but insufficient log entry propagation.}
        \label{fig:leadercompl-cex-a}
    \end{subfigure}\\

    %%% Figure B.
    \begin{subfigure}[b]{0.98\textwidth}
        \centering
        \input{figures/cex-tikz/leadercompl-no-term-check}
        \caption{Safety counterexample generated after disabling precondition Q2. Proper log entry propagation, but insufficient term deactivation.}
        \label{fig:leadercompl-cex-b}
    \end{subfigure}

    \caption{\textit{LeaderCompleteness} counterexamples generated by TLC. Primary servers are annotated with a \textcolor{blue}{\symqueen}. The state violating the safety property is highlighted in red. \mytodo{Adjust formatting to make figure width fit easily on page.} \mytodo{Explain server state representation.} \mytodo{Mark committed entries in traces.}}
    
    % Explain state representation.
    % $\underset{cfg}{S^T_{(v,t)}}$
\end{figure}

==> figures/mongo-legacy-reconfig-pseudocode.tex <==
\renewcommand{\algorithmicprocedure}{\textbf{action:}}

% \begin{minipage}{\dimexpr.5\textwidth-.5\columnsep}
\begin{algorithm}
    \caption{Pseudocode of \textit{MongoLegacyReconfig} reconfiguration specific behavior.}
    \label{alg:mrr-pseudocode}
    \begin{multicols}{2}
    \begin{algorithmic}[1]
    \small

    % TODO: Consider condensing variable names for pseudocode description.

    %%% States.
    \State \underline{\textbf{State and Initialization}}\\\\

    Let $C_{init} \in \mathcal{P}(Server) \setminus \emptyset$\\
    For all $i \in Server:$ \\
    \ \ $currentTerm_i \in \mathbb{N}$, initially $0$\\
    \ \ $state_i \in \{Primary, Secondary\}$, \\ \ \ \ initially $Secondary$\\
    \ \ $config_i \in \mathcal{P}(Server)$, initially $C_{init}$\\
    \ \ $configVersion_i \in \mathbb{N}$, initially $1$
    \columnbreak
    %%% Transitions.
    \State \underline{\textbf{Actions}}\\

    \Procedure{Reconfig}{i, newConfig} 
    % \Comment{Primary $i$ executes a reconfiguration.}
    \State Precondition:
    % \State \ \ $C(i)$ is committed
    \State \ \ $state_i = Primary$.
    \State \ \ $QuorumsOverlap(config_i, newConfig)$.
    \State Effect:
    \State \ \ $config_i \gets newConfig$.
    \State \ \ $configVersion_i \gets configVersion_i + 1$.

    \EndProcedure
    \\

    \Procedure{SendConfig}{i,j} 
    % \Comment{Server $i$ sends its newer config to server $j$. }
    \State Precondition:
    \State \ \ $state_j = Secondary$
    \State \ \ $C(i) > C(j)$
    \State Effect:
    \State \ \ $C(j) \gets C(i)$
    \EndProcedure
    \\

    % \Procedure{BecomeLeader}{i} 
    % % \Comment{Server $i$ becomes a primary.}
    % \State Precondition:
    % \State \ \ $\exists Q \in Quorums(config_i)$ : all $v \in Q$ cast votes for $i$ and $i \in Q$
    % \State Effect:
    % \State \ \ $state_i \gets Primary$
    % \State \ \ $state_j \gets Secondary$, $\forall j \in (Q \setminus \{i\})$
    % \State \ \ $currentTerm_i \gets currentTerm_i + 1$
    % \State \ \ $configTerm_i \gets currentTerm_i + 1$
    % \EndProcedure
    % \\

    % \Procedure{UpdateTerms}{i,j} 
    % % \Comment{Server $i$ sends server $j$ its newer term.}
    % \State Precondition:
    % \State \ \ $currentTerm_i > currentTerm_j$
    % \State Effect:
    % \State \ \ $state_j \gets Secondary$
    % \State \ \ $currentTerm_j \gets currentTerm_i$
    % \EndProcedure

    \end{algorithmic}
    \end{multicols}
\end{algorithm}
% \end{minipage}\hfill%



% \end{figure}

==> figures/mrr-protocol-tla-summary.tex <==
 \begin{figure}
    \captionsetup[subfigure]{justification=centering}
    \small
\begin{subfigure}[t]{0.40\textwidth}
    \input{tla-specs/tla-mongo-static-raft-next}
    % \caption{Variables and actions of \textit{MongoStaticRaft}}
    \caption{}
    \label{fig:msr-tla-next}
    \end{subfigure}
    \hspace{0.5cm}
    \begin{subfigure}[t]{0.55\textwidth}
    \input{tla-specs/tla-mongo-logless-dynamic-raft-next}
    % \caption{Variables and actions of \textit{MongoLoglessDynamicRaft}}
    \caption{}
    \label{fig:mldr-tla-next}
    \end{subfigure}
    
    \begin{subfigure}[t]{0.96\textwidth}
    \input{tla-specs/tla-mongo-raft-reconfig-next}
    % \caption{Variables and actions of \textit{MongoRaftReconfig}}
    \caption{}
    \label{fig:mrr-tla-next}
    \end{subfigure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

     \caption{The \textit{MongoRaftReconfig} transition relation defined as a composition of its subprotocols, \textit{MongoStaticRaft} and \textit{MongoLoglessDynamicRaft}. Actions in blue represent those of \textit{MongoStaticRaft}, and actions in orange represent those of \textit{MongoLoglessDynamicRaft}. The UNCHANGED construct indicates that a set of variables do not change on a transition.}
     \label{fig:mrr-composition}
     %TODO: If need to condense overall space in paper, consider changing 'currentTerm' to 'term'
\end{figure}
